Finding Smallest Witnesses for Conjunctive Queries

A witness is a sub-database that preserves the query results of the original database but of much smaller size. It has wide applications in query rewriting and debugging, query explanation, IoT analytics, multi-layer network routing, etc. In this paper, we study the smallest witness problem (SWP) for the class of conjunctive queries (CQs) without self-joins. We first establish the dichotomy that SWP for a CQ can be computed in polynomial time if and only if it has {\em head-cluster property}, unless $\texttt{P} = \texttt{NP}$. We next turn to the approximated version by relaxing the size of a witness from being minimum. We surprisingly find that the {\em head-domination} property - that has been identified for the deletion propagation problem \cite{kimelfeld2012maximizing} - can also precisely capture the hardness of the approximated smallest witness problem. In polynomial time, SWP for any CQ with head-domination property can be approximated within a constant factor, while SWP for any CQ without such a property cannot be approximated within a logarithmic factor, unless $\texttt{P} = \texttt{NP}$. We further explore efficient approximation algorithms for CQs without head-domination property: (1) we show a trivial algorithm which achieves a polynomially large approximation ratio for general CQs; (2) for any CQ with only one non-output attribute, such as star CQs, we show a greedy algorithm with a logarithmic approximation ratio; (3) for line CQs, which contain at least two non-output attributes, we relate SWP problem to the directed steiner forest problem, whose algorithms can be applied to line CQs directly. Meanwhile, we establish a much higher lower bound, exponentially larger than the logarithmic lower bound obtained above. It remains open to close the gap between the lower and upper bound of the approximated SWP for CQs without head-domination property.

==> macros.tex <==
\newcommand{\numtables}{{p}}
\newcommand{\allattr}{{\mathbb A}}
\newcommand{\aval}{{\mathbb a}}
\newcommand{\attrset}{{\mathbb B}}
\newcommand{\valset}{{\mathbb b}}
\newcommand{\allrel}{{\mathbb R}}
\newcommand{\queryattr}{{\mathcal A}}
\newcommand{\attr}{{\texttt{attr}}}
\newcommand{\head}{{\texttt{head}}}
\newcommand{\rel}{{\texttt{rels}}}
\newcommand{\dom}{{\texttt{dom}}}
%%\newcommand{\ourprob}{{\texttt{GDP}}}
\newcommand{\true}{{\texttt{true}}}
\newcommand{\false}{{\texttt{false}}}
\newcommand{\isptime}{{\textsc{IsPtime}}}
\newcommand{\caseempty}{{\texttt{{\bf EmptyQuery-1}}}} %{{\texttt{Simplify-1-EmptyQuery}}}
%%\newcommand{\casesingle}{{\texttt{\bf SingleRelation-2}}}
%{{\texttt{Simplify-2-SingleRelation}}}
%%\newcommand{\casetwo}{{\texttt{\bf TwoRelations-3}}}
%{{\texttt{Simplify-3-TwoRelations}}}
\newcommand{\casesubset}{{\texttt{\bf Subset-3}}}
%{{\texttt{Simplify-4-Subset}}}
\newcommand{\casecommon}{{\texttt{\bf CommonAttribute-4}}}
%{{\texttt{Simplify-5-CommonAttribute}}}
%%\newcommand{\casecooccur}{{\texttt{\bf CoOccurrence-6}}}
%{{\texttt{Simplify-6-CoOccurrence}}}
\newcommand{\casedecompose}{{\texttt{\bf Decomposition-5}}}
\newcommand{\caseboolean}{{\texttt{\bf Boolean-2}}}
%{{\texttt{Simplify-7-Decomposition}}}
\newcommand{\rectree}{{{recursion-tree}}}

\newcommand{\optcost}{{\textsc{OptCost}}}
\newcommand{\optsol}{{\textsc{OptSol}}}

\newcommand{\ceil}[1]{{\lceil #1 \rceil}}


\newcommand{\computeopt}{{\textsc{ComputeOpt}}}
\newcommand{\singlerel}{{\textsc{SingleRelation}}}
\newcommand{\tworel}{{\textsc{TwoRelations}}}
\newcommand{\onesubset}{{\textsc{OneSubset}}}
\newcommand{\commonattr}{{\textsc{CommonAttrPartition}}}
\newcommand{\cooccur}{{\textsc{CoOccurrence}}}
\newcommand{\decompose}{{\textsc{DecompCrossProduct}}}
\newcommand{\onedominant}{{\textsc{OneDominant}}}
\renewcommand{\boolean}{{\textsc{Boolean}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% COMMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ZM}[1]{\todo[inline]{\textbf{Zhengjie says:$\,$} #1}}
\newcommand{\JY}[1]{\todo[inline]{\textbf{Jun says:$\,$} #1}}
\newcommand{\SR}[1]{\todo[inline]{\textbf{Sudeepa says:$\,$} #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{black}{rgb}{0,0,0}
\definecolor{grey}{rgb}{0.8,0.8,0.8}
\definecolor{red}{rgb}{1,0,0}
\definecolor{green}{rgb}{0,1,0}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkpurple}{rgb}{0.5,0,0.5}
\definecolor{darkdarkpurple}{rgb}{0.3,0,0.3}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{shadegreen}{rgb}{0.95,1,0.95}
\definecolor{shadeblue}{rgb}{0.95,0.95,1}
\definecolor{shadered}{rgb}{1,0.85,0.85}
\definecolor{shadegrey}{rgb}{0.85,0.85,0.85}
\definecolor{oddRowGrey}{rgb}{0.80,0.80,0.80}
\definecolor{evenRowGrey}{rgb}{0.85,0.85,0.85}

\newcommand{\scream}[1]{{\textbf{\tt #1}}}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}\newcommand{\cut}[1]{{}}

\newcommand{\revm}[1]{#1} %{{\color{red} #1}}
\newcommand{\reva}[1]{#1} %{{\color{blue} #1}}
\newcommand{\revb}[1]{#1} %{{\color{darkgreen} #1}}
\newcommand{\revc}[1]{#1} %{{\color{darkpurple} #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Examples
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% STRUCTURE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mypar}[1]{\smallskip\noindent\textbf{{#1}.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% THEOREM LIKE ENVIRONMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathAlphabet{\mathbbold}{U}{bbold}{m}{n}

\cut{
\newtheorem{Theorem}{Theorem}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{Lemma}{Lemma}
\newtheorem{Proposition}{Proposition}
\theoremstyle{example}
\newtheorem{example}{Example}[section]
}

\newtheorem{theorem}{Theorem}[section]          	% Theorem environment.
\newaliascnt{lemma}{theorem}				% 1 alias counter
\newtheorem{lemma}[lemma]{Lemma}              	% Lemma environment.
\aliascntresetthe{lemma}  					% 3 set
\newaliascnt{conjecture}{theorem}			% 1 alias counter
\newtheorem{conjecture}[conjecture]{Conjecture}    % Conjecture environment.
\aliascntresetthe{conjecture}  				% 3 set
\newaliascnt{remark}{theorem}				% 1 alias counter
\newtheorem{remark}[remark]{Remark}              
\aliascntresetthe{remark}  					% 3 set
\newaliascnt{corollary}{theorem}			% 1 alias counter
\newtheorem{corollary}[corollary]{Corollary}      % Corollary environment.
\aliascntresetthe{corollary}  				% 3 set
\newaliascnt{definition}{theorem}			% 1 alias counter
\newtheorem{definition}[definition]{Definition}    % Definition environment.
\aliascntresetthe{definition}  				% 3 set
\newaliascnt{proposition}{theorem}			% 1 alias counter
\newtheorem{proposition}[proposition]{Proposition}  % proposition environment.
\aliascntresetthe{proposition}  				% 3 set
\newaliascnt{example}{theorem}			% 1 alias counter
\newtheorem{example}[example]{Example}  	% 2 environment.
\aliascntresetthe{example}  				% 3 set
\newaliascnt{observation}{theorem}			% 1 alias counter
\newtheorem{observation}[observation]{Observation}  % proposition environment.
\aliascntresetthe{observation}  				% 3 set
%\newtheorem{observation}[observation]{Observation}      % Corollary environment.
%\aliascntresetthe{observation}  				% 3 set
%\newtheorem{observation}{Observation}


\providecommand{\observationautorefname}{Obs.}
\providecommand{\definitionautorefname}{Definition}
\providecommand{\exampleautorefname}{Example}
\providecommand{\corollaryautorefname}{Corollary}
\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Section}


\newcommand{\proofpara}[1]{\medskip\noindent\underline{{#1}:}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% MATH UTILS AND STANDARD OPERATORS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mathtext}[1]{\ensuremath{\,\text{#1}\,}}
\newcommand{\card}[1]{|{#1}|}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\powset}[1]{\mathcal{P}(#1)}
\DeclareMathOperator*{\defas}{:=}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% COMPLEXITY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\oNotation}{O}
\newcommand{\NPhard}{NP-hard}
\newcommand{\NPcomplete}{NP-complete}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RUNNING EXAMPLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\egTup}{\tup_0}
\newcommand{\egQ}{\query_0}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% EXPERIMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\theRADB}{the relational algebra interpreter}
\newcommand{\aRADB}{a relational algebra interpreter}
\newcommand{\OurSys}{\textsc{RATest}}
\newcommand{\provBasic}{\textsc{Prov-All}}
\newcommand{\provSP}{\textsc{Prov-SP}}
\newcommand{\solverBasic}{\textsc{Solver-Naive}}
\newcommand{\solveOpt}{\textsc{Solver-Opt}}
\newcommand{\spjudBasic}{\textsc{Basic}}
\newcommand{\spjudOpt}{\textsc{$Opt_{\sigma}$}}
% \newcommand{\aggBasic}{\textsc{Agg-Basic}}
% \newcommand{\aggParam}{\textsc{Agg-Param}}
% \newcommand{\aggHeu}{\textsc{Agg-Opt}}
\newcommand{\aggBasic}{\textsc{AGG-base}}
\newcommand{\aggParam}{\textsc{AGG-base}}
\newcommand{\aggHeu}{\textsc{AGG-impr}}

\newcommand{\SCPall}{\textsc{SCP-all}}
\newcommand{\SCPsel}{\textsc{SCP-sel}}
\newcommand{\SAT}[1]{\textsc{SAT*#1}}
\newcommand{\SMT}{\textsc{SMT}}
\newcommand{\AGGbase}{\textsc{AGG-base}}
\newcommand{\AGGimpr}{\textsc{AGG-impr}}


\newcommand{\Vavg}{\mathfrak{avg}}
\newcommand{\Vsum}{\mathfrak{sum}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% REL MODEL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\schema}{S}
\newcommand{\schemaOf}[1]{{\sc {#1}}}
\newcommand{\relschema}{s}
\newcommand{\uDom}{\mathcal{U}}
\newcommand{\arity}[1]{arity({#1})}
\newcommand{\db}{D}
\newcommand{\makeRel}[1]{\textsf{#1}}
\newcommand{\query}{Q}
\newcommand{\qClass}{\mathcal{C}}
\newcommand{\tup}{t}
\newcommand{\multip}{n}
\newcommand{\aDom}{\mathbb{D}}
\newcommand{\aVal}{d}



\newcommand{\eg}{{e.g.}}
\newcommand{\ie}{{i.e.}}
\newcommand{\constraints}{{\Gamma}}
\newcommand{\witset}{{\mathcal W}}
\newcommand{\SCP}{{\tt SCP}}
\newcommand{\SWP}{{\tt SWP}}
\newcommand{\PAns}{{\mathcal A}}
\newcommand{\Prv}{{\tt Prv}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algebra
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\selection}{\sigma}
\newcommand{\projection}{\pi}
\newcommand{\join}{\Join}
\newcommand{\union}{\cup}
\newcommand{\intersection}{\cap}
\newcommand{\difference}{-}
\newcommand{\rename}{\rho}
\newcommand{\aggregation}[2]{\gamma_{{\tt #1, #2}}}  %{{}_{#1}\gamma_{#2}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../antiprov_main"
%%% End:

